Spherically symmetric elastic bodies in general relativity

The purpose of this review it to present a renewed perspective of the problem of self-gravitating elastic bodies under spherical symmetry. It is also a companion to the papers [Phys. Rev. D105, 044025 (2022)], [Phys. Rev. D106, L041502 (2022)], and [arXiv:2306.16584 [gr-qc]], where we introduced a new definition of spherically symmetric elastic bodies in general relativity, and applied it to investigate the existence and physical viability, including radial stability, of static self-gravitating elastic balls. We focus on elastic materials that generalize fluids with polytropic, linear, and affine equations of state, and discuss the symmetries of the energy density function, including homogeneity and the resulting scale invariance of the TOV equations. By introducing invariant characterizations of physical admissible initial data, we numerically construct mass-radius-compactness diagrams, and conjecture about the maximum compactness of stable physically admissible elastic balls.

==> table.tex <==
% \begin{table}[]
% \begin{tabular}{|l|l|l|l|}
% \hline
% \textbf{Acronym} & \textbf{Model}            & \textbf{Reference} & \textbf{Features}                                                                                                                                    \\ \hline
% QP               & Quadratic                 & Sec.~\ref{sec:QM}                & \begin{tabular}[c]{@{}l@{}}Deformation of polytropic fluid EoS,\\ XXX \end{tabular} \\ \hline
% NSI              & Newtonian Scale Invariant & Sec.~\ref{NSI}                & \begin{tabular}[c]{@{}l@{}}Scale invariant in the Newtonian limit,\\ XXXX   \end{tabular} \\ \hline
% LIS              & Linear Isotropic State    & Sec.~\ref{LIS}                & \begin{tabular}[c]{@{}l@{}}Scale invariant, pre-stressed, \\ deformation of linear fluid EoS\\ Constant wave speeds at the isotropic state\end{tabular} \\ \hline
% AIS              & Affine Isotropic State    & Sec.~\ref{AIS}                & \begin{tabular}[c]{@{}l@{}}Stress-free, deformation of affine fluid EoS\\ Constant wave speeds at the isotropic state\end{tabular}                   \\ \hline
% CLSF             & XXX                       & Sec.~\ref{CLSF}                & Stress-free, constant longitudinal wave speed                                                                                                         \\ \hline
% CLPS             & XXXX                      & Sec.~\ref{CLPS}               & Pre-stressed, constant longitudinal wave speed                                                                                                        \\ \hline
% \end{tabular}\label{table}
% \caption{Summary table of the elastic material models considered in this work.}
% \end{table}



\begin{table}[]
\begin{tabular}{|c|l|c|l|}
\hline
\textbf{Acronym} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{Reference} & \multicolumn{1}{c|}{\textbf{Features}}  \\ \hline
QP               & Quadratic                           & Sec.~\ref{sec:QM}                 
& \begin{tabular}[c]{@{}l@{}}Generalisation of polytropic fluid EoS:\\ - pre-stressed reference state, \\
- simplest model \end{tabular}   \\ \hline
NSI              & Newtonian Scale Invariant           & Sec.~\ref{NSI}                 
& \begin{tabular}[c]{@{}l@{}}Generalisation of polytropic fluid EoS: \\ - pre-stressed reference state, \\ - scale invariant in the Newtonian limit, \\ - includes quadratic model with $\mathrm{n}=1$ \end{tabular}  \\ \hline
LIS              & Linear Isotropic State              & Sec.~\ref{LIS}                
& \begin{tabular}[c]{@{}l@{}} Generalisation of linear fluid EoS: \\  - pre-stressed reference state \\ - relativistic scale invariant, \\ - constant wave speeds at the isotropic state\end{tabular} \\ \hline
AIS              & Affine Isotropic State              & Sec.~\ref{AIS}                
& \begin{tabular}[c]{@{}l@{}} Generalisation of affine fluid EoS: \\
- stress-free reference state, \\ - constant wave speeds at the isotropic state\end{tabular}  \\ \hline
ACS             & Affine Constant Speed                                & Sec.~\ref{ACS}                 
& \begin{tabular}[c]{@{}l@{}} Generalisation of affine fluid EoS: \\
- stress-free reference state, \\ - constant longitudinal wave speeds \end{tabular}            \\ \hline
LCS             & Linear Constant Speed                                & Sec.~\ref{LCS}                
&  \begin{tabular}[c]{@{}l@{}} Generalisation of linear fluid EoS: \\ 
- pre-stressed reference state, \\ - constant longitudinal wave speeds \end{tabular}             \\ \hline
\end{tabular}\label{table}
\caption{Summary table of the elastic material models considered in this work.
}
\end{table}
